Quantum Electrometer for Time-Resolved Material Science at the Atomic Lattice Scale

The detection of individual charges plays a crucial role in fundamental material science and the advancement of classical and quantum high-performance technologies that operate with low noise. However, resolving charges at the lattice scale in a time-resolved manner has not been achieved so far. Here, we present the development of an electrometer with 60 ns acquisition steps, leveraging on the spectroscopy of an optically-active spin defect embedded in a solid-state material with a non-linear Stark response. By applying our approach to diamond, a widely used platform for quantum technology applications, we can distinguish the distinct charge traps at the lattice scale, quantify their impact on transport dynamics and noise generation, analyze relevant material properties, and develop strategies for material optimization.

==> latexmkrc <==
# This shows how to use the xr package with latexmk.
# John Collins 2023-03-29
#
# The xr package ("a system for eXternal References") is used by a document
# to make references to sections, equations, etc in other external
# documents. 
# The definitions in this file enable latexmk to apply latexmk to
# automatically update an external document whenever its .tex file changes,
# so that the references in the main document stay up to date.

# Notes:
#    1. This version is defined to put the files from the compilations of
#       the external documents into a defined subdirectory, to segregate
#       potentially many generated files from the main document
#       directories. 
#    2. But for latexmk's custom dependency mechanism to be used, as here,
#       the aux file from compilation of a subdocument must be generated in
#       the same directory as the corresponding source .tex file.  So the
#       .aux file is copied.
#    3. It is assumed that the external documents are to be compiled by
#       pdflatex.  This can be changed, of course, by changing the '-pdf'
#       option given to the invoked latexmk to whatever is needed.
#    4. An ideal implementation would also ensure that recompilation of an
#       external document also happens whenever any of its other source
#       files changes.  But this is not done in the present version, and
#       would probably entail either the use of internal latexmk variables
#       or extra enhancements to latexmk.
#    5. The code uses subroutines copy and fileparse that are loaded by
#       latexmk from the Perl packages File::Copy and File::Basename.
#    6. It also uses some not-yet-documented features of latexmk: an array
#       variable @file_not_found and subroutines popd, pushd, and
#       rdb_add_generated. 


#--------------------
# Configurable choices for compilation of external documents

# Subdirectory for output files from compilation of external documents:
$sub_doc_output = 'output-subdoc';

# Options to supply to latexmk for compilation of external documents:
@sub_doc_options = ();

push @sub_doc_options, '-pdf'; # Use pdflatex for compilation of external documents.
# Replace '-pdf' by '-pdfdvi', 'pdfxe', or 'pdflua' if needed.

#--------------------

# Add a pattern for xr's log-file message about missing files to latexmk's
# list.  Latexmk's variable @file_not_found is not yet documented.
# This line isn't necessary for v. 4.80 or later of latexmk.
push @file_not_found, '^No file\\s*(.+)\s*$';

add_cus_dep( 'tex', 'aux', 0, 'makeexternaldocument' );
sub makeexternaldocument {
    if ( $root_filename ne $_[0] )  {
        my ($base_name, $path) = fileparse( $_[0] );
        pushd $path;
        my $return = system "latexmk",
                            @sub_doc_options,
                            "-aux-directory=$sub_doc_output",
                            "-output-directory=$sub_doc_output",
                            $base_name;
        if ( ($sub_doc_output ne ' ') && ($sub_doc_output ne '.') ) {
               # In this case, .aux file generated by pdflatex isn't in same
               # directory as the .tex file.
               # Therefore:
               # 1. Actual generated aux file must be listed as produced by this
               #    rule, so that latexmk deals with dependencies correctly.
               #    (Problem to overcome: If $sub_dir_output is same as $aux_dir
               #    for the main document, xr may read the .aux file in the
               #    aux_dir rather than the one the cus dep is assumed by latexmk
               #    to produce, which is in the same directory as the .tex source
               #    file for this custom dependency.)
               #    Use not-yet-documented latexmk subroutine rdb_add_generated
               #    to do this:
               # 2. A copy of the .aux file must be in same directory as .tex file
               #    to satisfy latexmk's definition of a custom dependency.
             rdb_add_generated( "$sub_doc_output/$base_name.aux" );
             copy "$sub_doc_output/$base_name.aux", ".";
        }
        popd;
        return $return;
   }
}

==> preamble.tex <==

\usepackage{graphicx}
\usepackage[usenames,dvipsnames]{xcolor}
\usepackage{amssymb,amsfonts,amsmath}
\usepackage[colorlinks=true,citecolor=Cerulean,linkcolor=RubineRed,urlcolor=Cerulean]{hyperref}
\usepackage{epstopdf}
\usepackage{bm}
\usepackage{bbold}
\usepackage{upgreek}
\usepackage[inline]{enumitem}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage[normalem]{ulem}
\usepackage{IEEEtrantools}
\usepackage{makecell}
\renewcommand\theadfont{}
\usepackage{tabularx}
\usepackage{float}

\usepackage{afterpage}
\newcommand\blankpage{%
    \null
    \thispagestyle{empty}%
    \addtocounter{page}{-1}%
    \newpage}

\usepackage{verbatim}
\newcommand{\detailtexcount}[1]{%
  \immediate\write18{texcount -merge -sum -q #1.tex output.bbl > #1.wcdetail }%
  \verbatiminput{#1.wcdetail}%
}
\newcommand{\quickwordcount}[1]{%
  \immediate\write18{texcount -1 -sum -merge -q #1.tex output.bbl > #1-words.sum }%
  \input{#1-words.sum} words%
}
\newcommand{\quickcharcount}[1]{%
  \immediate\write18{texcount -1 -sum -merge -char -q #1.tex output.bbl > #1-chars.sum }%
  \input{#1-chars.sum} characters (not including spaces)%
}


\usepackage{babel}
\usepackage{lipsum}
\usepackage{sidecap}
\usepackage{hyperref}
\hypersetup{
    colorlinks=true,
    linkcolor=magenta,
    filecolor=magenta,      
    urlcolor=cyan
    }

    
\usepackage{xr}
\makeatletter
\newcommand*{\addFileDependency}[1]{
  \typeout{(#1)}
  \@addtofilelist{#1}
  \IfFileExists{#1}{}{\typeout{No file #1.}}
}
\makeatother
\newcommand*{\myexternaldocument}[1]{%
    \externaldocument{#1}%
    \addFileDependency{#1.tex}%
    \addFileDependency{#1.aux}%
}



\newcommand{\im}{\mathrm{i}}
\newcommand{\kBT}{k_\mathrm{B}T}
\newcommand{\kB}{k_\mathrm{B}}
\newcommand{\ud}{\mathrm{d}}
\newcommand{\bv}[1]{{\boldsymbol #1}}
\newcommand{\ket}[1]{\left|#1\right\rangle}
\newcommand{\bra}[1]{\left\langle #1\right|}
\newcommand{\ketbra}[2]{\left|#1\right\rangle \left\langle #2 \right|}
\renewcommand{\vec}[1]{\mathbf{#1}}
\newcommand{\gtwo}{\textsl{g}^2}
\newcommand{\EXP}[1]{~\times~10^{#1}}
\newcommand{\Ang}{${\rm \AA ngstr\ddot{o}m}$}



\usepackage{txfonts}
\usepackage{latexsym}


\newcommand{\tosupp}[1]{{\color{ForestGreen}{\bf SUPP}: {\em #1}}}
\newcommand{\tocut}[1]{{\color{BrickRed}{\bf CUT}: \sout{#1}}}
\newcommand{\todo}[1]{{\color{DarkOrchid} $\{\{${\bf TODO}: #1$\}\}$}}
\newcommand{\jhdm}[1]{{\color{PineGreen}$\langle\langle$#1$\rangle\rangle$}}
\newcommand{\cgt}[1]{{\color{Maroon}#1}}
\newcommand{\gp}[1]{{\color{NavyBlue}#1}}
\newcommand{\ts}[1]{{\color{Lavender}#1}}
\newcommand{\cg}[1]{{\color{RubineRed}#1}}

\graphicspath{ {./figz/} }

% \usepackage[style=nature]{biblatex}
% \addbibresource{refz.bib} 

%\bibliographystyle{apsrev4-2}
% \bibliographystyle{naturemag}

%\usepackage{natbib}
% \usepackage[super,numbers]{natbib}

\setcitestyle{super} \bibliographystyle{naturemag_manual}
\makeatletter 
\renewcommand\bibnumfmt[1]{{#1.}}
\makeatother 
\def\bibsection{\section*{\refname}} 
\newcommand*{\citen}[1]{%
  \begingroup
  \romannumeral-`\x % remove space at the beginning of 
    \setcitestyle{numbers,open={},close={}}
    \cite{#1}%
  \endgroup   
}

% \usepackage[backend=biber,
%   style=nature,
%   sorting=none,
%   giveninits=true,
%   isbn=false,doi=false,url=false,
%   natbib=true
% ]{biblatex}

% \DeclareFieldFormat{journaltitle}{#1\isdot}
% \DeclareFieldFormat[article,periodical]{volume}{#1\isdot}

% \addbibresource{refz.bib}

\newlist{custominlist}{enumerate*}{1}
\setlist[custominlist]{label=(\roman*)}

==> title.tex <==
\title{Quantum Electrometer for Time-Resolved Material Science at the Atomic Lattice Scale}

\author{Gregor Pieplow}
\altaffiliation{These authors contributed equally to this work}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}

\author{Cem G\"{u}ney Torun}
\altaffiliation{These authors contributed equally to this work}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}

\author{Charlotta Gurr}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}

\author{Joseph H. D. Munns}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}

\author{Franziska Marie Herrmann}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}

\author{Andreas Thies}
\affiliation{Ferdinand-Braun-Institut (FBH), Gustav-Kirchhoff-Str. 4, 12489 Berlin, Germany}

\author{Tommaso Pregnolato}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}
\affiliation{Ferdinand-Braun-Institut (FBH), Gustav-Kirchhoff-Str. 4, 12489 Berlin, Germany}

\author{Tim Schr\"{o}der}
\email[Corresponding author: ]{tim.schroeder@physik.hu-berlin.de}
\affiliation{Department of Physics, Humboldt-Universit\"{a}t zu Berlin, 12489 Berlin, Germany}
\affiliation{Ferdinand-Braun-Institut (FBH), Gustav-Kirchhoff-Str. 4, 12489 Berlin, Germany}

